Beyond a Global Norm: Personalizing Toxicity Sensitivity in Language Models Without Retraining

Reducing toxicity is often framed as a global alignment problem, yet perceptions of harmful language are subjective and context-dependent. We present the first comparative evaluation of training-free methods for aligning language generation to user-specific toxicity sensitivities across three inference-time intervention stages: pre-decoding (prompt conditioning and rewriting), in-decoding (token, logit, and representation steering), and post-decoding (candidate re-ranking). Evaluated against toxicity sensitivity targets derived from the PRISM dataset, all methods reduce alignment error by 28-47%. However, the results reveal a fundamental trade-off between alignment effectiveness, personalization, and general language quality, showing how toxicity sensitivity alignment is an inherently multi-objective problem.

==> Sections/results_old.tex <==
\section{Results}
We report results using the benchmark's comparative questions: whether each stage improves toxicity-profile alignment, whether the improvement reflects personalisation rather than a generic safe shift, and what trade-offs each stage introduces. Across stages, the central pattern is that training-free interventions can move model outputs closer to PRISM-derived user toxicity targets without modifying model weights. However, the mechanism and cost of this movement differ substantially by intervention stage.

\subsection{All intervention stages improve toxicity-profile alignment}
All four intervention families reduce distance to the PRISM-preferred toxicity profile relative to their unsteered baselines, but they do so with different levels of consistency and stage-specific constraints. Pre-decoding methods show that substantial alignment gains are possible with input-only access. URIAL-inspired prompt conditioning produces the strongest pre-decoding results, improving toxicity-distance by 50.56\% on Llama and 30.94\% on Qwen. PBPO-Lite prompt rewriting also improves over the base condition, but to a lesser extent: 24.39\% on Llama and 15.63\% on Qwen. This suggests that low-access personalisation can be effective, but preserving the original prompt while adding guidance is more stable than rewriting it.

\begin{figure}[h]
\small
\centering
\begin{tikzpicture}
\begin{axis}[
width=\columnwidth,
height=5cm,
ylabel=MAE reduction (\%),
ybar,
ymin=0, ymax=60,
ytick={0,10,20,30,40,50,60},
xtick={0,1,2},
xticklabels={URIAL, Classifier, Manhattan, Mahalanobis},
x tick label style={rotate=25,anchor=east},
bar width=14pt,
enlarge x limits=0.3,
legend pos=north east,
legend cell align={left},
legend columns=1,
ymajorgrids=true,
grid style=dashed,
]
% pre-decoding
\addplot [
        pink,fill=pink!30!white,postaction={pattern=horizontal lines},
        error bars/.cd, y dir=both, y explicit,
    ] table[x={x}, y={y}, y error={error}] {
        x y error
        0 50.56 0
    }; \addlegendentry{pre-decoding}
    % in-decoding classifier
\addplot [
        magenta,fill=magenta!30!white,postaction={pattern=vertical lines},
        error bars/.cd, y dir=both, y explicit,
    ] table[x={x}, y={y}, y error={error}] {
        x y error
        1 33.55 0
    }; \addlegendentry{classifier-decoding}
% post-decoding (real, seeds 1/13/21, n=600)
\addplot [
        violet,fill=violet!30!white,postaction={pattern=dots},
        error bars/.cd, y dir=both, y explicit,
    ] table[x={x}, y={y}, y error={error}] {
        x y error
        2 31.2 3.9
        3 28.5 3.9
    }; \addlegendentry{post-decoding}
\end{axis}
\end{tikzpicture}
\caption{Average MAE reduction per method.}
\label{fig:MAE}
\end{figure}


\begin{figure*}[h]
\small
\centering
\begin{tikzpicture}
\begin{axis}[
width=2\columnwidth,
height=5cm,
ylabel=Sensitivity score,
ybar,
ymin = -0.8, ymax = 0.2,
xtick={0,1,2,3,4,5},
xticklabels={Toxicity, Severe toxicity, Identity attack, Insult, Profanity, Threat},
x tick label style={rotate=25,anchor=east},
bar width=6pt,
enlarge x limits=0.1,
legend pos=south east,
legend cell align={left},
legend columns=7,
legend style={/tikz/every even column/.append style={column sep=0.2cm}},
ymajorgrids=true,
grid style=dashed,
]
\addplot [pink,fill=pink!30!white,postaction={pattern=horizontal lines}] table[x={point}, y={URIAL}] {tikz/MAE_categories.dat};
\addplot [purple,fill=purple!30!white,postaction={pattern=vertical lines}] table[x={point}, y={method_1}] {tikz/MAE_categories.dat};
\addplot [violet,fill=violet!30!white,postaction={pattern=dots}] table[x={point}, y={method_2}] {tikz/MAE_categories.dat};
\addplot [teal,fill=teal!30!white,postaction={pattern=grid}] table[x={point}, y={method_3}] {tikz/MAE_categories.dat};
\addplot [black,fill=cyan!30!white,postaction={pattern=north east lines}] table[x={point}, y={Manhattan}] {tikz/MAE_categories.dat};
\addplot [magenta,fill=magenta!30!white,postaction={pattern=crosshatch dots}] table[x={point}, y={Mahalanobis}] {tikz/MAE_categories.dat};
\legend{URIAL, method 1, Classifier, method 3, Manhattan, Mahalanobis}
\end{axis}
\end{tikzpicture}
\caption{Sensitivity reduction per category.}
\label{fig:MAE_categories}
\end{figure*}

Classifier-guided in-decoding consistently reduces toxicity error across the three held-out seeds, with improvements of 24.82\%, 41.80\%, and 33.40\%. Aggregated over all 600 prompt-user records, this gives a 33.55\% improvement over the unguided baseline, with guided outputs improving over the baseline on 61.3\% of prompts. The largest gain appears on the more toxic \textit{harmful-borderline} prompts, where MAE improves by 36.82\%, compared to \textit{benign} prompts, which improve by 26.36\%.

Representation-level steering shows a sharper operating range. Population CAA reduces toxicity MAE from 0.02149 to 0.01478 at $\alpha=0.3$, corresponding to a 31.2\% drop, with the strongest improvements concentrated on harmful-borderline and safe-sensitive prompt categories. However, increasing steering strength beyond the productive range quickly degrades generation quality, indicating that representation steering is powerful but calibration-sensitive.

Post-decoding re-ranking reduces error most consistently across scorer variants. All four re-ranking modules reduce mean chosen MAE from the baseline of 0.0198 to between 0.01420 and 0.01520, corresponding to 23.3--28.4\% improvement. The top three scorers---GPT judge, weighted Manhattan, and Claude judge---are effectively tied, with differences smaller than seed-to-seed variation. This suggests that, for post-decoding selection, a cheap deterministic geometric matcher can perform comparably to expensive LLM-as-a-Judge re-ranking.

\subsection{Personalisation is visible only under user-sensitive evaluations}
Aggregate toxicity-distance reduction alone does not show whether an intervention is genuinely personalised. A method may improve by shifting all outputs toward lower toxicity, even if it does not respond to the individual user profile. The benchmark, therefore, includes user-sensitive checks wherever possible.

\begin{figure}[h]
\small
\centering
\begin{tikzpicture}
\begin{axis}
[
width=\columnwidth,
height=6cm,
xlabel=MMLU accuracy (\%),
ylabel=Mean toxicity improvement (\%)
]
\addplot[
    only marks,
    mark=*,
    mark options={fill=red},
    nodes near coords=URIAL
] coordinates {(25.7,35.9)};

\addplot[
    only marks,
    mark=*,
    mark options={fill=blue},
    nodes near coords={method 1}
] coordinates {(25.8,42.7)};

\addplot[
    only marks,
    mark=*,
    mark options={fill=green},
    nodes near coords={Classifier}
] coordinates {(65.7,33.55)};

\addplot[
    only marks,
    mark=*,
    mark options={fill=orange},
    nodes near coords={method 3}
] coordinates {(26.1,21.0)};

\addplot[
    only marks,
    mark=*,
    mark options={fill=purple},
    nodes near coords={method 4}
] coordinates {(20.3,41.7)};

\addplot[
    only marks,
    mark=*,
    mark options={fill=black},
    nodes near coords={method 5}
] coordinates {(22.5,42.9)};

\end{axis}
\end{tikzpicture} 
\caption{MMLU vs. toxicity reduction.}
\label{fig:MMLU}
\end{figure}

\begin{figure}[h]
\small
\centering
\begin{tikzpicture}
\begin{axis}[
width=\columnwidth,
height=6cm,
xlabel=Perplexity (lower is better),
ylabel=Mean toxicity improvement (\%),
clip=false,
enlarge x limits=0.12,
enlarge y limits=0.15,
]
\addplot[only marks, mark=*, mark options={fill=cyan}, nodes near coords={Manhattan},
    every node near coord/.append style={anchor=west, xshift=3pt}] coordinates {(8.33,31.2)};
\addplot[only marks, mark=*, mark options={fill=magenta}, nodes near coords={Mahalanobis},
    every node near coord/.append style={anchor=west, xshift=3pt}] coordinates {(8.12,28.5)};
\addplot[only marks, mark=*, mark options={fill=red}, nodes near coords={URIAL},
    every node near coord/.append style={anchor=north, yshift=-3pt}] coordinates {(25.7,35.9)};
\addplot[only marks, mark=*, mark options={fill=blue}, nodes near coords={method 1},
    every node near coord/.append style={anchor=west, xshift=3pt}] coordinates {(25.8,42.7)};
\addplot[only marks, mark=*, mark options={fill=green}, nodes near coords={Classifier},
    every node near coord/.append style={anchor=south, yshift=3pt}] coordinates {(5.7,33.55)};
\addplot[only marks, mark=*, mark options={fill=orange}, nodes near coords={method 3},
    every node near coord/.append style={anchor=south, yshift=3pt}] coordinates {(26.1,21.0)};
\addplot[only marks, mark=*, mark options={fill=purple}, nodes near coords={method 4},
    every node near coord/.append style={anchor=east, xshift=-3pt}] coordinates {(20.3,41.7)};
\addplot[only marks, mark=*, mark options={fill=black}, nodes near coords={method 5},
    every node near coord/.append style={anchor=south, yshift=3pt}] coordinates {(22.5,42.9)};
\end{axis}
\end{tikzpicture} 
\caption{MMLU vs. fluency.}
\label{fig:perplexity}
\end{figure}

In pre-decoding, the personalisation signal is present but uneven. URIAL improves by 50.56\% with personalised examples, compared with 41.13\% under an instruction-only ablation, giving a 9.43 percentage-point personalisation gap. PBPO-Lite shows a smaller gap: 24.39\% improvement with the matched profile versus 22.75\% with a shuffled profile. This suggests that input-level personalisation contributes to improvement, but that much of the gain may also come from generic safety conditioning or rewriting.

Classifier-guided decoding provides stronger evidence of directional personalisation. Because the toxicity penalty is weighted by each user's six-dimensional sensitivity vector, we can test whether the categories reduced by the decoder align with the user's profile. The median per-user cosine alignment is 0.845, significantly above a shuffled-weight baseline ($p=0.0097$). This shows that the decoder is not merely lowering toxicity globally but also reducing the categories to which a given user is most sensitive.

Representation steering shows a related distinction between population-level and user-level metrics. Population CAA achieves the lowest toxicity MAE, but the per-user compositional arms perform best on preference prediction accuracy: dislike-weighted composition reaches 59.9\%, ideal-point composition 55.3\%, compared with 54.3\% for the population direction. This reversal indicates that standard toxicity MAE can reward proximity to a population target, while preference-sensitive metrics better capture movement toward individual users' preferred responses.

Post-decoding re-ranking offers the clearest isolation test because the same candidate pool can be re-ranked under different user profiles. Profile-shuffle tests show that selections respond to the matched user rather than to any arbitrary profile. The effect is also visible in boundary-violation metrics, whereas aggregate mean error can mask per-user differences. This is a methodological result of the benchmark: personalised alignment requires evaluation metrics that preserve the user as the unit of analysis.

\subsection{The main trade-offs are stage-specific}
The interventions differ less in whether they can reduce toxicity-distance than in what they trade away to do so. Pre-decoding is the lowest-access strategy but also the most vulnerable to task-format interference. URIAL preserves the original prompt and yields strong gains in toxicity, yet MMLU results show that safety-prefixing can still distract from structured knowledge tasks, especially on Llama. PBPO-Lite is more expressive because it uses the full six-dimensional profile, but rewriting can alter the wording of the task or the answer structure. This is reflected in large drops on MMLU, particularly for Qwen under PBPO-Lite and for Llama under both pre-decoding interventions.

Classifier-guided decoding preserves utility more reliably. All three methods remain within 0.7 percentage points of the unguided MMLU baseline and increase perplexity only minimally. The main cost is runtime: because the guidance classifier scores top-$k$ candidate tokens at every decoding step, throughput drops from 30.6 tokens/sec in the unguided baseline to roughly 13--15 tokens/sec at the main operating point $k=20$. Thus, classifier guidance offers directional control with limited loss of capability, but at a clear decoding-time cost.

Representation steering introduces no prompt overhead and does not require candidate re-ranking, but it comes at the cost of calibration stability. At low steering strengths, CAA improves alignment while preserving utility; zero-shot MMLU remains within noise. At higher strengths, perplexity increases sharply, and generations can collapse into repetitive strings. Per-user composition partly improves the fluency--alignment balance, but it also shows that activation-space personalisation is sensitive to vector norms, basis construction, and the reliability of the user signal.

Post-decoding re-ranking is the most auditable stage. Candidate responses, scores, and final selections can be inspected, and the same pool can be reused for profile-shuffle tests. Its cost lies in candidate generation and, for LLM judges, scorer expense and stochasticity. It also depends on candidate diversity: re-ranking can only select a better response if the base model generated one. The strongest gains, therefore, occur with harmful-borderline prompts, where the candidate pool exhibits greater variation and the baseline is farther from the user target. On benign-control prompts, where all candidates are already near-zero toxicity, re-ranking has little room to improve.

%\subsection{Summary of comparative findings}
% Taken together, the results show that personalised toxicity alignment can be implemented at multiple points in the inference pipeline, but each stage affords a different kind of control. Pre-decoding is cheap and broadly deployable, but indirect and vulnerable to task interference. Classifier-guided decoding provides directional token-level control, with modest fluency and utility costs but substantial throughput overhead. Representation steering offers internal control without prompt overhead, but requires white-box access and careful calibration to avoid generation collapse. Post-decoding re-ranking is auditable and effective, but bounded by candidate diversity and selection cost.

% The benchmark, therefore, does not identify a single universally best stage. Instead, it shows that the intervention stage determines what kind of personalisation is possible, how it can be verified, and which costs must be managed. This supports the central claim of the paper: personalised alignment is not only a question of which objective to optimise, but where in the generation pipeline user-specific information should enter.pink
